Modulated bimaximal neutrino mixing

The present article is an endeavor to look into some fruitful frameworks based on "Bi-maximal" neutrino mixing, from a model independent stand. The possibilities involving the correction or attenuation of the original BM mixing matrix, followed by GUT-inspired charged lepton correction are invoked. The "symmetry-basis" thus constructed, accentuates some interesting facets such as: a modified QLC relation, $\theta_{12}+\theta_{c}\approx\frac{\pi}{4}-\theta_{13}\cos(n\pi-\delta_{CP})$, a possible link up between neutrino and charged lepton sectors, $\theta_{13}^{\nu}=\theta_{12}^{l}\sim\mathcal{O}(\theta_{C})$ or that between neutrinos and quarks, $\theta_{13}^{\nu}=\theta_{C}$. The study vindicates the relevance of the Bi-maximal mixing as a first approximation.

==> Table1.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{l}
\hline
\hline
\vspace{0.1 cm}
{\footnotesize $\mathcal{A}\approx -f^2 s \epsilon ^4+f^2 s \epsilon ^3-s \epsilon ^4+s \epsilon ^2+\epsilon ^2$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{B}\approx -\frac{1}{2} d^2 f s \epsilon ^4-d s \epsilon ^4-\frac{d \epsilon ^4}{2}+d \epsilon ^2-\frac{1}{2} f^3 s \epsilon ^4-\frac{1}{2} f s \epsilon ^4-f s \epsilon ^3+f s \epsilon ^2$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{C}\approx -\frac{d^2 \epsilon ^3}{2}+d f s \epsilon ^4-d f s \epsilon ^3-f^2 s \epsilon ^4-s \epsilon ^3-\frac{\epsilon ^3}{2}+\epsilon $ }\\ 
\vspace{0.1 cm} 
{\footnotesize $\mathcal{D}\approx -d^2 s \epsilon ^3-d^2 \epsilon ^4+d^2 \epsilon ^2-2 d f s \epsilon ^4+f^2 s \epsilon ^4-f^2 s \epsilon ^3+s \epsilon$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{E}\approx \frac{1}{2} d^3 s \epsilon ^4-\frac{d^3 \epsilon ^3}{2}+d f^2 s \epsilon ^4-d s \epsilon ^2-d \epsilon ^3+d \epsilon +f s \epsilon ^4-f s \epsilon ^3$} \\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{F}\approx d^2 s \epsilon ^3+d^2 \epsilon ^4-d^2 \epsilon ^2+2 d f s \epsilon ^4+s \epsilon ^4+\frac{\epsilon ^4}{4}-\epsilon ^2+1$} \\ 
\hline 
\end{tabular} 
\caption{\label{table1} The elements of the general neutrino mass matrix (Normal Hierarchy-non-degenerate (\textbf{NH-ND}) case)}
\end{center}
\end{table*}


==> Table2.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{l}
\hline
\hline
\vspace{0.1 cm}
{\footnotesize $\mathcal{A}\approx b^2 \gamma ^2+\frac{c^2 \eta ^2}{3}+\frac{2}{3} c \eta ^2 c'^2$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{B}\approx -\frac{1}{3} \eta  \{b \gamma  \left(c^2 \eta ^2-3\right)+2 b c \gamma  \eta ^2 c'^2+\sqrt{2} (c-1) c \eta  \kappa  c'\}$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{C}\approx \frac{1}{3} \{b \gamma  \kappa  \left(3-c^2 \eta ^2\right)-2 b c \gamma  \eta ^2 \kappa c'^2+\sqrt{2} (c-1) c \eta ^3 c'\}$ }\\ 
\vspace{0.1 cm} 
{\footnotesize $\mathcal{D}\approx \frac{1}{9} \eta ^2 \{c \left(\sqrt{6} b \gamma  \eta  c'+\sqrt{3} c \kappa \right)^2+3 \left(b c \gamma  \eta -\sqrt{2} \kappa  c'\right)^2+9\}$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{E}\approx-\frac{1}{3} \eta  \{-2 \eta ^2 \kappa  \left(c'\right)^2 \left(b^2 c \gamma ^2-1\right)+\kappa  \left(-b^2 \gamma ^2 c^2 \eta ^2+c^3 \eta ^2-3\right)+\sqrt{2} b (c-1) c \gamma  \eta  c' \left(\eta ^2-\kappa ^2\right)\}$} \\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{F}\approx \frac{1}{9} \eta ^2 \left(\sqrt{3} b c \gamma  \kappa +\sqrt{6} \eta  c'\right)^2+\frac{1}{9} c \eta ^2 \left(\sqrt{3} c \eta -\sqrt{6} b \gamma  \kappa  c'\right)^2+\kappa ^2$} \\ 
\hline 
\end{tabular} 
\caption{\label{table2} The elements of the general neutrino mass matrix (\textbf{NH-QD} case) }
\end{center}
\end{table*}

==> Table3.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{l}
\hline
\hline
\vspace{0.1 cm}
{\footnotesize $\mathcal{A}\approx b^2 \gamma ^2 \eta ^2+\frac{c^2}{3}+\frac{2}{3} c c'^2$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{B}\approx -\frac{1}{3} b c^2 \gamma  \eta -\frac{2}{3} b c \gamma  \eta  c'^2+b \gamma  \eta ^3+\frac{1}{3} \sqrt{2} c \kappa  c'-\frac{1}{3} \sqrt{2} c^2 \kappa  c'$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{C}\approx -\frac{1}{3} b \gamma  c^2 \kappa -\frac{2}{3} b \gamma  c \kappa c'^2+b \gamma  \eta ^2 \kappa -\frac{1}{3} \sqrt{2} c \eta  c'+\frac{1}{3} \sqrt{2} c^2 \eta  c'$ }\\ 
\vspace{0.1 cm} 
{\footnotesize $\mathcal{D}\approx \frac{1}{3} b^2 c^2 \gamma ^2 \eta ^2+\frac{2}{3} b^2 c \gamma ^2 \eta ^2 c'^2-\frac{2}{3} \sqrt{2} b c \gamma  \eta  \kappa  c'+\frac{1}{3} \sqrt{2} 2 b c^2 \gamma  \eta  \kappa  c'+\frac{c^3 \kappa ^2}{3}+\frac{2}{3} \kappa ^2 c'^2+\eta ^4$ }\\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{E}\approx\frac{1}{3} b^2 \gamma ^2 c^2 \eta  \kappa +\frac{2}{3} b^2 \gamma ^2 c \eta  \kappa c'^2+\frac{1}{3} \sqrt{2} b \gamma  c \eta ^2 c'-\frac{1}{3} \sqrt{2} b \gamma  c \kappa ^2 c'-\frac{1}{3} \sqrt{2} b \gamma  c^2 \eta ^2 c'+\frac{1}{3} \sqrt{2} b \gamma  c^2 \kappa ^2 c'-\frac{1}{3} c^3 \eta  \kappa -\frac{2}{3} \eta  \kappa  c'^2+\eta ^3 \kappa$} \\ 
\vspace{0.1 cm}
{\footnotesize $\mathcal{F}\approx \frac{1}{3} b^2 \gamma ^2 c^2 \kappa ^2+\frac{2}{3} b^2 \gamma ^2 c \kappa ^2 c'^2+\frac{1}{3} \sqrt{2} 2 b \gamma  c \eta  \kappa  c'-\frac{2}{3} \sqrt{2} b \gamma  c^2 \eta  \kappa  c'+\frac{c^3 \eta ^2}{3}+\frac{2}{3} \eta ^2 c'^2+\eta ^2 \kappa ^2$} \\ 
\hline 
\end{tabular} 
\caption{\label{table3} The elements of the general neutrino mass matrix (\textbf{IH-QD} case)}
\end{center}
\end{table*}

==> Table4.tex <==
\begin{table*}
\setlength{\tabcolsep}{1 em}
\begin{center}
\begin{tabular}{l|c|c|c}
\hline 
\hline\\
 & {\footnotesize \textbf{Parameters} }& {\footnotesize \textbf{Prediction}} & {\footnotesize \textbf{Texture}} \\ 
\hline 
\hline\\
{\footnotesize \textbf{NH-ND}} & \begin{tabular}{l}
$\epsilon = 0.151859$,\\ 
$f=3.53882$, \\ 
$d=4.96783$, \\  
$s=1.21652$ ,\\ 
$m_{3}=0.0483055\,eV$. \\ 
\end{tabular}  & \begin{tabular}{l}
$m_{1}=0.00135518\,eV$,\\ 
$m_{2}=0.00892393\,eV$, \\ 
$\Delta\,m_{21}^2= 7.78\times 10^{-5}\,eV^{2}$, \\ 
$\Delta\,m_{31}^2=2.33\times 10^{-3}\,eV^{2}$,\\ 
$\sin^2\theta_{12}=0.289$, \\ 
$\sin^2\theta_{23}= 0.569$, \\ 
$\sin^2\theta_{13}=0.0233$, \\ 
$\Sigma\,m_{i}=0.0585846 \,eV$. \\ 
\end{tabular}  & 
\begin{tabular}{l}
$\begin {bmatrix}\mathcal {A} & 2 \,\mathcal {A} - \mathcal {C} & \
\mathcal {C} \\ 2\,\mathcal {A} - \mathcal {C} & 6\,\mathcal {A} + \mathcal {C} & 4\, \
\mathcal {A} + \mathcal {C} \\ \mathcal {C} & 4\, \mathcal {A} + \
\mathcal {C} & 5\, \mathcal {A} + \mathcal {C} \\
\end {bmatrix}m_{3}$\\ 
\\
\begin{scriptsize}
%% modified nh.nb
$\mathcal{A}=0.0946855$,\,\, $\mathcal{C}=0.038355$.
\end{scriptsize}
\end{tabular}
\\
\\
{\footnotesize \textbf{NH-QD}} & \begin{tabular}{l}
\begin{tabular}{l}
$\eta=0.762386$ ,\\ 
$b=1.56568$,\\ 
$c=0.96663$,\\ 
$m_{3}=0.0588\,eV$. \\ 
\end{tabular}  \\ 
\\
\\
\begin{tabular}{l}
$\eta= 0.756875$, \\ 
$b=1.4945$,\\ 
$c=0.96663$, \\ 
$m_{3}=0.0588\,eV$. \\ 
\end{tabular}  \\ 
\end{tabular}   & \begin{tabular}{l}
\begin{tabular}{l}
$m_{1}=0.0330417\,eV$,\\ 
$m_{2}=0.0341791\,eV$, \\ 
$\Delta\,m_{21}^2= 7.65\times 10^{-5}\,eV^{2}$, \\ 
$\Delta\,m_{31}^2=2.37\times 10^{-3}\,eV^{2}$,\\ 
$\sin^2\theta_{12}=0.315$, \\ 
$\sin^2\theta_{23}= 0.581$, \\ 
$\sin^2\theta_{13}=0.0319$, \\ 
$\Sigma\,m_{i}=0.126036 \,eV$. \\ 
\end{tabular} \\ 
\\
\\
\begin{tabular}{l}
$m_{1}=0.0325638\,eV$,\\ 
$m_{2}=0.0336859\,eV$, \\ 
$\Delta\,m_{21}^2= 7.43\times 10^{-5}\,eV^{2}$, \\ 
$\Delta\,m_{31}^2=2.40\times 10^{-3}\,eV^{2}$,\\ 
$\sin^2\theta_{12}=0.314$, \\ 
$\sin^2\theta_{23}= 0.573$, \\ 
$\sin^2\theta_{13}=0.0259$, \\ 
$\Sigma\,m_{i}=0.12506 \,eV$. \\ 
\end{tabular}  \\ 
\end{tabular}  & \begin{tabular}{l}
$\begin {bmatrix}
\mathcal {A} & \mathcal {B} &\frac{2}{3}\mathcal{B}\\
 \mathcal {B} & 4 \mathcal {E} & \mathcal {E} \\
\frac{2}{3}\mathcal{B} & \mathcal {E} & 4 \mathcal {E} - \mathcal {B} \\
\end{bmatrix}m_{3}$
\\
\\ 
\begin{scriptsize}
$\mathcal{A}=0.581819$,\,\, $\mathcal{B}=0.0636482$,\end{scriptsize}\\
\begin{scriptsize}
$\mathcal{E}=0.203162$.
\end{scriptsize}
\\
\\
\\
$\begin {bmatrix} 
\mathcal {A} & \mathcal {B} &\frac {2 } {3} \mathcal{B} \\ 
\mathcal {B} & \mathcal {D} &\mathcal {E} \\
\frac {2 }{3}\mathcal {B} &\mathcal {E} & \mathcal {D} - \mathcal {B} \\
\end{bmatrix}m_{3}$\\ 
\\ 
\begin{scriptsize}
$\mathcal{A}=0.571196 $,\,\, $\mathcal{B}=0.058653 $,\end{scriptsize}\\
\begin{scriptsize}
$\mathcal{D}=0.80716$,\,\, $ \mathcal{E}=0.208885$. %%modifications.nb
\end{scriptsize}
\end{tabular} \\
\hline 
\\
{\footnotesize \textbf{IH-QD}} & \begin{tabular}{l}
\begin{tabular}{l}
$\eta=0.774459$,\\ 
$b=0.950921$,\\ 
$c=0.989598$, \\ 
$m_{2}=0.0612\,eV$. \\ 
\end{tabular}  \\ 
\\
\\
\begin{tabular}{l}
$\eta= 0.761187$, \\ 
$b=1.31518$,\\ 
$c=0.989553$, \\ 
$m_{3}=0.06047\,eV$. \\ 
\end{tabular}  \\ 
\end{tabular} & \begin{tabular}{l}
\begin{tabular}{l}
$m_{1}=0.0605614\,eV$,\\ 
$m_{3}=0.0367071\,eV$, \\ 
$\Delta\,m_{21}^2= 7.75\times 10^{-5}\,eV^{2}$, \\ 
$\Delta\,m_{31}^2=2.32\times 10^{-3}\,eV^{2}$,\\ 
$\sin^2\theta_{12}=0.3264$, \\ 
$\sin^2\theta_{23}= 0.599$, \\ 
$\sin^2\theta_{13}=0.0151$, \\ 
$\Sigma\,m_{i}=0.158464 \,eV$. \\ 
\end{tabular}\\ 
\\
\\
\begin{tabular}{l}
$m_{1}=0.0598426\,eV$,\\ 
$m_{3}=0.0350405\,eV$, \\ 
$\Delta\,m_{21}^2= 7.57\times 10^{-5}\,eV^{2}$, \\ 
$\Delta\,m_{31}^2=2.35\times 10^{-3}\,eV^{2}$,\\ 
$\sin^2\theta_{12}=0.3264$, \\ 
$\sin^2\theta_{23}= 0.579$, \\ 
$\sin^2\theta_{13}=0.0219$, \\ 
$\Sigma\,m_{i}=0.155355\,eV$. \\ 
\end{tabular}  \\ 
\end{tabular}   & \begin{tabular}{l}
$\begin {bmatrix} 
\mathcal {A} &\mathcal {B} & \mathcal {B} \\ 
\mathcal {B} &\mathcal { 
      D} &\mathcal {D} - \mathcal {A} - \mathcal {B} \\ 
B &\mathcal {D} - \mathcal {A} - \mathcal {B} &  \mathcal {F} \\
\end {bmatrix}m_{2}$ \\
\\ 
\begin{scriptsize}
$\mathcal{A}= 0.987095,\,\,\mathcal{B}=-0.0341297$
\end{scriptsize}\\
\begin{scriptsize}
$\mathcal{D}=0.761603 ,\,\mathcal{F}=0.840778$.
\end{scriptsize} %% modifications.nb
\\
\\
$\begin {bmatrix} 
\mathcal {A} &\mathcal {B} & \mathcal {B} \\ 
\mathcal {B} &\mathcal { 
      D} &\mathcal {F} - \mathcal {A} + \mathcal {B} \\ 
B &\mathcal {F} - \mathcal {A} + \mathcal {B} &  \mathcal {F} \\
\end {bmatrix}m_{2}$\\
\\ 
\begin{scriptsize}
$\mathcal{A}= 0.983997,\,\,\mathcal{B}=-0.0430051$
\end{scriptsize}\\
\begin{scriptsize}
$\mathcal{D}=0.759459 ,\,\mathcal{F}=0.825692$,
\end{scriptsize} %% modifications.nb
\end{tabular}  \\ 
\hline 
\end{tabular}
\caption{\label{table4}\footnotesize The summary of parametrization and the neutrino mass matrix texture}
\end{center} 
\end{table*}

==> Table5.tex <==
\begin{table*}
\setlength{\tabcolsep}{1 em}
\begin{center}
\begin{tabular}{l||l}
\hline
\hline\\
\vspace{0.1 cm}
\textbf{I} & \begin{tabular}{l}$
\mathcal{A}\underbrace{\begin{bmatrix}
0 & 2 & 0\\
2 & 6 & 4\\
0 & 4 & 5
\end{bmatrix}}+
\mathcal{C}\left\lbrace\underbrace{\begin{bmatrix}
0 & 0 & 1\\
0 & 1 & 0\\
1 & 0 & 0
\end{bmatrix}} + \underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & 1\\
0 & 1 & 0
\end{bmatrix}}+ \underbrace{\begin{bmatrix}
0 & -1 & 0\\
-1 & 0 & 0\\
0 & 0 & 1
\end{bmatrix}}\right\rbrace+(\mathcal{A-C})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 0
\end{bmatrix}}$\\
$\hspace{0.83 cm}H\hspace{1.9cm} f_{1} \hspace{1.455 cm} d_{1}\hspace{1.63cm} e_{4}\hspace{3.15 cm} T_{1}$
\end{tabular}\\
\hline\\
\textbf{II} &\begin{tabular}{l}$
(\mathcal{E-B})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & 1\\
0 & 1 & 0
\end{bmatrix}}+
(4\mathcal{E}-B)\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 1 & 0\\
0 & 0 & 1
\end{bmatrix}} + \mathcal{B}\underbrace{\begin{bmatrix}
1 & 1 & 1\\
1 & 1 & 1\\
1 & 1 & 1
\end{bmatrix}}+(\mathcal{A}-5\mathcal{E}+\frac{10}{9}\mathcal{B})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 0
\end{bmatrix}} + \mathcal{B}\underbrace{\begin{bmatrix}
-\frac{1}{9} & 0 & -\frac{1}{3}\\
0 & 0 & 0\\
-\frac{1}{3} & 0& -1 
\end{bmatrix}}$\\
$\hspace{1.7 cm}d_{1} \hspace{1.6cm}  \hspace{1.07cm} I \hspace{1.7 cm} D\hspace{3.71cm} T_{1}\hspace{1.87 cm} T_{2}$
\end{tabular}\\
\hline\\
\textbf{III} &\begin{tabular}{l}$
(\mathcal{E-B})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & 1\\
0 & 1 & 0
\end{bmatrix}}+
(\mathcal{D}-B)\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 1 & 0\\
0 & 0 & 1
\end{bmatrix}} + \mathcal{B}\underbrace{\begin{bmatrix}
1 & 1 & 1\\
1 & 1 & 1\\
1 & 1 & 1
\end{bmatrix}}+(\mathcal{A}-\mathcal{E-D}+\frac{10}{9}\mathcal{B})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & 0\\
0 & 0 & 0
\end{bmatrix}} + \mathcal{B}\underbrace{\begin{bmatrix}
-\frac{1}{9} & 0 & -\frac{1}{3}\\
0 & 0 & 0\\
-\frac{1}{3} & 0& -1 
\end{bmatrix}}$\\
$\hspace{1.7 cm}d_{1} \hspace{1.6cm}  \hspace{0.99 cm} I \hspace{1.73 cm} D\hspace{4.15 cm} T_{1}\hspace{1.9 cm}T_{2}$
\end{tabular}\\
\hline\\
\textbf{IV} &\begin{tabular}{l}$
(\mathcal{A-D})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & -1\\
0 & -1 & 0
\end{bmatrix}}
- \mathcal{B}\left\lbrace\underbrace{\begin{bmatrix}
0 & -1 & 0\\
0 & 0 & 1\\
-1 & 0 & 0
\end{bmatrix}}+\underbrace{\begin{bmatrix}
0 & 0 & -1\\
-1 & 0 & 0\\
0 & 1 & 0
\end{bmatrix}}\right\rbrace+\mathcal{D}\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 1 & 0\\
0 & 0 & \frac{\mathcal{F}}{\mathcal{D}}
\end{bmatrix}}$\\
$\hspace{2.05 cm}d_{2} \hspace{2.4 cm} c_{3} \hspace{2 cm} b_{3}\hspace{2.29 cm} T_{3}$
\end{tabular}\\
\hline\\
\textbf{V} &\begin{tabular}{l}$
(\mathcal{A-F})\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 0 & -1\\
0 & -1 & 0
\end{bmatrix}}
+ \mathcal{B}\left\lbrace\underbrace{\begin{bmatrix}
1 & 1 & 1\\
1 & 1 & 1\\
1 & 1 & 1
\end{bmatrix}}-\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & 1 & 0\\
0 & 0 & 1
\end{bmatrix}}\right\rbrace+\mathcal{F}\underbrace{\begin{bmatrix}
1 & 0 & 0\\
0 & \frac{\mathcal{D}}{\mathcal{F}} & 0\\
0 & 0 & 1
\end{bmatrix}}$\\
$\hspace{2.04cm}d_{2} \hspace{2.12 cm}D \hspace{1.48 cm} I \hspace{2.25 cm} T_{4}$
\end{tabular}\\
\\
\hline
\end{tabular} 
\caption{\label{table5} The expression of \textbf{Textures I-V}, in terms of corresponding building block matrices}
\end{center}
\end{table*}
